QDGset: A Large Scale Grasping Dataset Generated with Quality-Diversity

Recent advances in AI have led to significant results in robotic learning, but skills like grasping remain partially solved. Many recent works exploit synthetic grasping datasets to learn to grasp unknown objects. However, those datasets were generated using simple grasp sampling methods using priors. Recently, Quality-Diversity (QD) algorithms have been proven to make grasp sampling significantly more efficient. In this work, we extend QDG-6DoF, a QD framework for generating object-centric grasps, to scale up the production of synthetic grasping datasets. We propose a data augmentation method that combines the transformation of object meshes with transfer learning from previous grasping repertoires. The conducted experiments show that this approach reduces the number of required evaluations per discovered robust grasp by up to 20%. We used this approach to generate QDGset, a dataset of 6DoF grasp poses that contains about 3.5 and 4.5 times more grasps and objects, respectively, than the previous state-of-the-art. Our method allows anyone to easily generate data, eventually contributing to a large-scale collaborative dataset of synthetic grasps.

==> tex_files/appendices.tex <==




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                       Supplementary materials
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\clearpage
\appendices

\input{tex_files/tables/qdg_set_details}
\input{tex_files/figures/appendix_boxplot_details_sample_efficiency}




==> tex_files/figures/visualization_augmented_object_ycb_chips_can.tex <==



\begin{figure}[t]
  \centering
\centering
  \includegraphics[width=\columnwidth]{assets/ycb_chips_can_100_augmentation_samples.png}
  \caption{\textbf{3D meshes augmentation.} In red is the reference YCB chips can, and in grey a subsample of 100 resulting augmentations.}
  \label{fig:vis_augment_ycb_chips_can}
\end{figure}


==> tex_files/tables/qdg_set_details.tex <==




\begin{table*}[t]
\centering
\begin{tabular}{ || c || c | c | c | c | c | c ||}

\hline

\makecell{\textbf{Objects source}} & \makecell{\textbf{Num.}\\\textbf{objects}}  & \makecell{\textbf{Num.}\\\textbf{grasps}} & \makecell{\textbf{Mean grasps}\\\textbf{per object}}  & \makecell{\textbf{Std grasps}\\\textbf{per object}} & \makecell{\textbf{Num.}\\\textbf{no success}} & \makecell{\textbf{Objects type}} \\

\hhline{||=||=|=|=|=|=|=||}

3DNet & 1\,175 & 4\,449\,168 & 3\,787 & 1\,621 & 0 & Daily (intermediate complexity: dishes, shoes, tools, keyboards, toys ...)  \\
\hline
KIT & 129 & 437\,380 & 3\,391  & 344 & 0 & Daily (simple: cylinders, boxes + some more complex objects)  \\
\hline
YCB & 94 & 145\,626 & 1\,549  & 1\,146 & 12 & Daily (intermediate complexity: dishes, tools, toys)  \\
\hline
Graspnet1Billion & 87 & 179\,887 & 2\,044 & 894 & 2 & Daily (intermediate complexity: dishes, tools, toys)  \\
\hline
ShapeNet & 25\,837 & 33\,214\,669 & 1\,286 & 1\,392 & 8\,691 & Human-scaled (high complexity: street and home furnitures, plumbing, vehicules, music instruments, ...) \\
\hline
EGAD & 2\,330 & 4\,604\,776 & 1\,977 & 395 & 0 & Adversarial  \\

\hhline{||=||=|=|=|=|=|=||}

3DNet\textit{-aug} & 9\,706 & 17\,018\,746 & 1\,753 & 1\,045 & 69 & Daily  \\
\hline
KIT\textit{-aug} & 1290 & 1\,527\,167 & 1\,535 & 359 & 0 & Daily  \\

\hhline{||=||=|=|=|=|=|=||}

\makecell{\textbf{Dataset}} & \makecell{\textbf{Num.}\\\textbf{objects}}  & \makecell{\textbf{Num.}\\\textbf{grasps}} & \makecell{\textbf{Mean grasps}\\\textbf{per object}} & \makecell{\textbf{Std grasps}\\\textbf{per object}} & \makecell{\textbf{Num.}\\\textbf{failures}} & \makecell{\textbf{Objects type}} \\

\hline

QDGSet\textit{-core} & 29\,652 & 43\,031\,506 & 1\,451 & 1\,446 & 8\,705 & Daily, human-scaled, adversarial  \\
\hline
QDGSet & 40\,648 & 61\,577\,419 & 1\,526 & 1\,348 & 8\,774 & Daily, human-scaled, adversarial  \\

\hline

\end{tabular}
\caption{\textbf{QDG-Set description.} Object sources with *-aug in their name corresponds to augmented object datasets. QDGSet\textit{-core} contains no augmented objects. QDGSet contains all the generated grasps on any kind of objects.}
\label{table:dataset_comparison_detailed}
\end{table*}


==> tex_files/tables/sim2real_deployment_results.tex <==


\begin{table}[t]
\centering
\begin{tabular}{ ||c || c | c | c  ||}
\hline
QD Framework & Reach-and-grasp & \multicolumn{2}{c||}{6DoF}   \\
\hline
Gripper & Panda & Panda & Allegro \\
\hline
 $\eta^{sim2real}$  & 0.84 & \textbf{0.95} & \textbf{0.72} \\
\hline

\end{tabular}
\caption{\textbf{Measured sim2real transfer ratios.}}
\label{table:s2r_deploy_results}
\end{table}


==> tex_files/tables/simulated_test_prediction_results.tex <==



\begin{table}[t]
\centering
\begin{tabular}{ ||c || c | c | c | c ||}
\hline
\textbf{Dex-Net dataset} & \textbf{Acc.} & \textbf{Prec.} & \textbf{Rec.} & \textbf{F1} \\ 
\hline
Vanilla \cite{mahler2017dexnet2} & \hl{...} & \hl{...} & \hl{...} & \hl{...}   \\
\hline
QDG6DoF + DR \cite{helenon2024learning}  & \hl{...} & \hl{...} & \hl{...} & \hl{...}  \\

\hhline{||=||=|=|=|=||}

QDGSet-\textit{core}  & \hl{...} & \hl{...} & \hl{...} & \hl{...}  \\
\hline
QDGSet-\textit{aug}  & \hl{...} & \hl{...} & \hl{...} & \hl{...}  \\

\hline


\end{tabular}
\caption{\textbf{Evaluation results of Dex-Net learning.}}
\label{table:evaluation_results_of_dexnet_learning}
\end{table}


